Embedding arbitrary Boolean circuits into fungal automata with arbitrary update sequences

The sandpile automata of Bak, Tang, and Wiesenfeld (Phys. Rev. Lett., 1987) are a simple model for the diffusion of particles in space. A fundamental problem related to the complexity of the model is predicting its evolution in the parallel setting. Despite decades of effort, a classification of this problem for two-dimensional sandpile automata remains outstanding. Fungal automata were recently proposed by Goles et al. (Phys. Lett. A, 2020) as a spin-off of the model in which diffusion occurs either in horizontal $(H)$ or vertical $(V)$ directions according to a so-called update scheme. Goles et al. proved that the prediction problem for this model with the update scheme $H^4V^4$ is $\textbf{P}$-complete. This result was subsequently improved by Modanese and Worsch (Algorithmica, 2024), who showed the problem is $\textbf{P}$-complete also for the simpler updatenscheme $HV$. In this work, we fill in the gaps and prove that the prediction problem is $\textbf{P}$-complete for any update scheme that contains both $H$ and $V$ at least once.

==> Figures/fig_sec_3_3/tik_semiwire_prom.tex <==
\begin{tikzpicture}[scale=.34]

    \draw[line width=0.1mm] (0, 6) grid (5, 10);

    \draw[line width=0.6mm] (0, 6) grid (0, 10);
    \draw[line width=0.6mm] (1, 6) grid (1, 10);
    \draw[line width=0.6mm] (2, 6) grid (2, 10);
    \draw[line width=0.6mm] (3, 6) grid (3, 10);
    \draw[line width=0.6mm] (4, 6) grid (4, 10);
    \draw[line width=0.6mm] (5, 6) grid (5, 10);

    \draw[line width=0.6mm] (0,10) -- (5,10);
    \draw[line width=0.6mm] (0,8) -- (5,8);
    \draw[line width=0.6mm] (0,6) -- (5,6);
    
    \setcounter{rows}{10}
    \setcounter{row}{0}
    \setrow {4,3,3,3,3}
    \setrow { ,3,3,3,3}
    \setrow { ,3,3,3,3}
    \setrow { , , , , };
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw (5,9.2) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,H)$};
\draw (13,9.2) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,V)$};
\draw (21,9.2) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,V)$};
\draw (29,9.2) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,H)$};

\draw (35,5.5) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,H)$};

\draw (5,3.2) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,V)$};
\draw (13,3.2) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,H)$};
\draw (21,3.2) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,V)$};
\draw (29,3.2) node [anchor=north west,scale=0.8][inner sep=0.75pt] {$F(\cdot,V)$};


\draw[- stealth] (5.2,8) -- (7.8,8);
\draw[- stealth] (13.2,8) -- (15.8,8);
\draw[- stealth] (21.2,8) -- (23.8,8);
\draw[- stealth] (29.2,8) -- (31.8,8);

\draw[- stealth] (34,5.8) -- (34,4.2);

\draw[- stealth] (7.8,2) -- (5.2,2);
\draw[- stealth] (15.8,2) -- (13.2,2);
\draw[- stealth] (23.8,2) -- (21.2,2);
\draw[- stealth] (31.8,2) -- (29.2,2);



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \draw[line width=0.1mm] (8, 6) grid (13, 10);

    \draw[line width=0.6mm] (8, 6) grid (8, 10);
    \draw[line width=0.6mm] (9, 6) grid (9, 10);
    \draw[line width=0.6mm] (10, 6) grid (10, 10);
    \draw[line width=0.6mm] (11, 6) grid (11, 10);
    \draw[line width=0.6mm] (12, 6) grid (12, 10);
    \draw[line width=0.6mm] (13, 6) grid (13, 10);
    
    \draw[line width=0.6mm] (8,10) -- (13,10);
    \draw[line width=0.6mm] (8,8) -- (13,8);
    \draw[line width=0.6mm] (8,6) -- (13,6);


    

    \setcounter{cols}{8}
    \setcounter{row}{0}
    \setrow {2,4,3,3,3}
    \setrow { ,3,3,3,3}
    \setrow { ,3,3,3,3}
    \setrow { , , , , };

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[line width=0.1mm] (16, 6) grid (21, 10);

\draw[line width=0.6mm] (16, 6) grid (16, 10);
\draw[line width=0.6mm] (17, 6) grid (17, 10);
\draw[line width=0.6mm] (18, 6) grid (18, 10);
\draw[line width=0.6mm] (19, 6) grid (19, 10);
\draw[line width=0.6mm] (20, 6) grid (20, 10);
\draw[line width=0.6mm] (21, 6) grid (21, 10);

\draw[line width=0.6mm] (16,10) -- (21,10);
\draw[line width=0.6mm] (16,8) -- (21,8);
\draw[line width=0.6mm] (16,6) -- (21,6);


    \setcounter{cols}{16}
    \setcounter{row}{0}
    \setrow {2,2,3,3,3}
    \setrow { ,4,3,3,3}
    \setrow { ,3,3,3,3}
    \setrow { , , , , };
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[line width=0.1mm] (32, 6) grid (37, 10);

\draw[line width=0.6mm] (32, 6) grid (32, 10);
\draw[line width=0.6mm] (33, 6) grid (33, 10);
\draw[line width=0.6mm] (34, 6) grid (34, 10);
\draw[line width=0.6mm] (35, 6) grid (35, 10);
\draw[line width=0.6mm] (36, 6) grid (36, 10);
\draw[line width=0.6mm] (37, 6) grid (37, 10);

\draw[line width=0.6mm] (32,10) -- (37,10);
\draw[line width=0.6mm] (32,8) -- (37,8);
\draw[line width=0.6mm] (32,6) -- (37,6);

    
\draw[line width=0.1mm] (24, 6) grid (29, 10);

\draw[line width=0.6mm] (24, 6) grid (24, 10);
\draw[line width=0.6mm] (25, 6) grid (25, 10);
\draw[line width=0.6mm] (26, 6) grid (26, 10);
\draw[line width=0.6mm] (27, 6) grid (27, 10);
\draw[line width=0.6mm] (28, 6) grid (28, 10);
\draw[line width=0.6mm] (29, 6) grid (29, 10);

\draw[line width=0.6mm] (24,10) -- (29,10);
\draw[line width=0.6mm] (24,8) -- (29,8);
\draw[line width=0.6mm] (24,6) -- (29,6);

    \setcounter{cols}{24}
    \setcounter{row}{0}
    \setrow {2,3,3,3,3}
    \setrow { ,2,3,3,3}
    \setrow { ,4,3,3,3}
    \setrow { , , , , };

    \setcounter{cols}{32}
    \setcounter{row}{0}
    \setrow {2,3,3,3,3}
    \setrow { ,2,3,3,3}
    \setrow {1,2,4,3,3}
    \setrow { , , , , };

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\draw[line width=0.1mm] (0, 0) grid (5, 4);

\draw[line width=0.6mm] (0, 0) grid (0, 4);
\draw[line width=0.6mm] (1, 0) grid (1, 4);
\draw[line width=0.6mm] (2, 0) grid (2, 4);
\draw[line width=0.6mm] (3, 0) grid (3, 4);
\draw[line width=0.6mm] (4, 0) grid (4, 4);
\draw[line width=0.6mm] (5, 0) grid (5, 4);

\draw[line width=0.6mm] (0,4) -- (5,4);
\draw[line width=0.6mm] (0,2) -- (5,2);
\draw[line width=0.6mm] (0,0) -- (5,0);

\setcounter{cols}{0}
\setcounter{rows}{4}
\setcounter{row}{0}
\setrow {2,3,3,3,3}
\setrow { ,2,4,3,3}
\setrow {1,2,2,3,3}
\setrow { , ,1, , };
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[line width=0.1mm] (8, 0) grid (13, 4);

\draw[line width=0.6mm] (8, 0) grid (8, 4);
\draw[line width=0.6mm] (9, 0) grid (9, 4);
\draw[line width=0.6mm] (10, 0) grid (10, 4);
\draw[line width=0.6mm] (11, 0) grid (11, 4);
\draw[line width=0.6mm] (12, 0) grid (12, 4);
\draw[line width=0.6mm] (13, 0) grid (13, 4);

\draw[line width=0.6mm] (8,4) -- (13,4);
\draw[line width=0.6mm] (8,2) -- (13,2);
\draw[line width=0.6mm] (8,0) -- (13,0);


\setcounter{cols}{8}
\setcounter{row}{0}
\setrow {2,3,4,3,3}
\setrow { ,2,2,3,3}
\setrow {1,2,3,3,3}
\setrow { , ,1, , };
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[line width=0.1mm] (16, 0) grid (21, 4);

\draw[line width=0.6mm] (16, 0) grid (16, 4);
\draw[line width=0.6mm] (17, 0) grid (17, 4);
\draw[line width=0.6mm] (18, 0) grid (18, 4);
\draw[line width=0.6mm] (19, 0) grid (19, 4);
\draw[line width=0.6mm] (20, 0) grid (20, 4);
\draw[line width=0.6mm] (21, 0) grid (21, 4);

\draw[line width=0.6mm] (16,4) -- (21,4);
\draw[line width=0.6mm] (16,2) -- (21,2);
\draw[line width=0.6mm] (16,0) -- (21,0);

\setcounter{cols}{16}
\setcounter{row}{0}
\setrow {2,4,2,4,3}
\setrow { ,2,2,3,3}
\setrow {1,2,3,3,3}
\setrow { , ,1, , };
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[line width=0.1mm] (32, 0) grid (37, 4);

\draw[line width=0.6mm] (32, 0) grid (32, 4);
\draw[line width=0.6mm] (33, 0) grid (33, 4);
\draw[line width=0.6mm] (34, 0) grid (34, 4);
\draw[line width=0.6mm] (35, 0) grid (35, 4);
\draw[line width=0.6mm] (36, 0) grid (36, 4);
\draw[line width=0.6mm] (37, 0) grid (37, 4);

\draw[line width=0.6mm] (32,4) -- (37,4);
\draw[line width=0.6mm] (32,2) -- (37,2);
\draw[line width=0.6mm] (32,0) -- (37,0);

\draw[line width=0.1mm] (24, 0) grid (29, 4);

\draw[line width=0.6mm] (24, 0) grid (24, 4);
\draw[line width=0.6mm] (25, 0) grid (25, 4);
\draw[line width=0.6mm] (26, 0) grid (26, 4);
\draw[line width=0.6mm] (27, 0) grid (27, 4);
\draw[line width=0.6mm] (28, 0) grid (28, 4);
\draw[line width=0.6mm] (29, 0) grid (29, 4);

\draw[line width=0.6mm] (24,4) -- (29,4);
\draw[line width=0.6mm] (24,2) -- (29,2);
\draw[line width=0.6mm] (24,0) -- (29,0);

\setcounter{cols}{24}
\setcounter{row}{0}
\setrow {2,2,2,2,3}
\setrow { ,3,2,4,3}
\setrow {1,2,3,3,3}
\setrow { , ,1, , };
\setcounter{cols}{32}
\setcounter{row}{0}
\setrow {2,2,2,3,3}
\setrow { ,3,2,2,3}
\setrow {1,2,3,4,3}
\setrow { , ,1, , };

\setcounter{cols}{0}
\end{tikzpicture}
